DeepLearningKit - an GPU Optimized Deep Learning Framework for Apple's iOS, OS X and tvOS developed in Metal and Swift

In this paper we present DeepLearningKit - an open source framework that supports using pretrained deep learning models (convolutional neural networks) for iOS, OS X and tvOS. DeepLearningKit is developed in Metal in order to utilize the GPU efficiently and Swift for integration with applications, e.g. iOS-based mobile apps on iPhone/iPad, tvOS-based apps for the big screen, or OS X desktop applications. The goal is to support using deep learning models trained with popular frameworks such as Caffe, Torch, TensorFlow, Theano, Pylearn, Deeplearning4J and Mocha. Given the massive GPU resources and time required to train Deep Learning models we suggest an App Store like model to distribute and download pretrained and reusable Deep Learning models.

==> memkitemetal.tex <==
This section gives short snippets of Metal code used as part deep learning (convolutional neural network) for the MNIST case.

\subsection{Parallel Convolution in Metal}
Each position (id) in the convolution output is calculated in parallel. Note that the version below is without striding support.

\begin{lstlisting}
  int y = id / conv_xdim;
  int x = id % conv_xdim;

  int mm,nn,ii,jj;

  // convolution
  for(int q=0; q<filter_ydim; ++q) {
    mm = filter_ydim-1-q;
    for(int r=0; r<filter_xdim; ++r) {
      nn = filter_xdim - 1 - r;
      ii = y + q;
      jj = x + r;
      convolution_output[id].real += image[ii*image_xdim+jj].real *
                       convolution_filter[mm*filter_xdim+nn].real;
    }
  }

  // ready to do max-pooling when all threads have appeared here
  threadgroup_barrier(mem_flags::mem_none);
\end{lstlisting}

\subsection{Parallel Max-Pooling Layer in Metal}
The max pooling output is calculated within the same layer as convolution in order to utilize parallelization, but is separated here for clarity.

\begin{lstlisting}
  // parallel calculation of 2x2 max-pooling
  if((y%2 == 0) && (x%2 == 0)) { // upper left corner of 2x2
    int pool_pos = int(y/2)*pool_xdim + int(x/2);
    float v1 = fmax(convolution_output[id].real,
                    convolution_output[id+1].real);
    float v2 = fmax(v1,
                    convolution_output[id+conv_xdim].real); 
    float max_pool_value = fmax(v2,
                    convolution_output[id+conv_xdim+1].real);
    pooling_output[pool_pos].real = tanh(max_pool_value + B);
  }
    
\end{lstlisting}

\subsection{Parallel Hidden Layer in Metal}
\begin{lstlisting}
  result[id] = b[id];
  for(int i=0; i<x_xdim; ++i) {
    result[id].real += X[id*x_xdim + i].real*w[i].real;
  }
  result[id].real = tanh(result[id].real);
\end{lstlisting}


\subsection{Parallel Logistic Regression Layer}
\begin{lstlisting}
  result[id] = b[id];
  for(int i=0; i<x_xdim; ++i) {
    result[id].real += X[id*x_xdim + i].real*w[i].real;
  }

  // finish calculation of result before continuing
  threadgroup_barrier(mem_flags::mem_none);
  int limit = result_xdim*result_ydim-1;

  float left, right;
  // recursive doubling calculation of softmax components
  for(int i=2; i<=limit; i*=2) {
    if(id % i == 0) {
      if(i == 2) { // first time
        left = result[id].real;
        right = result[id+i/2].real;
      } else {
        left = softmax[id].real;
        right = softmax[id+i/2].real;
      }
      softmax[id].real = fmax(left, right);
      array_sum[id].real = left + right;
    }
    // wait until all have calculated their part
    threadgroup_barrier(mem_flags::mem_none);
  }

  // if dimension is odd, also include the last object
  if(id == 0) {
    if(x_xdim*x_ydim % 2 != 0) {
      left = softmax[id].real;
      right = result[ x_xdim*x_ydim - 1].real;
      softmax[id].real = fmax(left,right);
      array_sum[id].real += right;
    }

    shared_max[id].real = softmax[id].real;
  }

  // all threads need to come here
  threadgroup_barrier(mem_flags::mem_none);

\end{lstlisting}

Parallel logistic regression in Metal continued.

  \begin{lstlisting}
  // ready to calculate e = exp(w-maxes)
  softmax[id].real = exp(softmax[id].real-shared_max[0].real);

  threadgroup_barrier(mem_flags::mem_none);

  for(int i=2; i<=limit; i*=2) {
    if(id % i == 0) {
      if(i == 2) {
        left = softmax[id].real;
        right = softmax[id+i/2].real;
      } else {
        left = array_sum[id].real;
        right = array_sum[id+i/2].real;
      }
      array_sum[id].real = left + right;
    }

    // wait until all have calculated their part
    threadgroup_barrier(mem_flags::mem_none);
   }

  // if dimension is odd, also include the last object
   if(id == 0) {
     if(x_xdim*x_ydim % 2 != 0) {
       left = array_sum[id].real;
       right = softmax[ x_xdim*x_ydim - 1].real;
       array_sum[id].real += right;
      }
   }

   threadgroup_barrier(mem_flags::mem_none);

   // ready to calculate dist = e/numpy.sum(e, axis=1)
   if(array_sum[id].real != 0.0) {
     softmax[id].real = softmax[id].real/array_sum[0].real;
   }
          
  \end{lstlisting}

  

  
  

